Accelerating LHC phenomenology with analytic one-loop amplitudes: A C++ interface to MCFM

The evaluation of one-loop matrix elements is one of the main bottlenecks in precision calculations for the high-luminosity phase of the Large Hadron Collider. To alleviate this problem, a new C++ interface to the MCFM parton-level Monte Carlo is introduced, giving access to an extensive library of analytic results for one-loop amplitudes. Timing comparisons are presented for a large set of Standard Model processes. These are relevant for high-statistics event simulation in the context of experimental analyses and precision fixed-order computations.

==> header.tex <==
%%%% AUTHORS
\usepackage{authblk}
% decrease font size in affiliation, see authblk
% documentation:
\renewcommand\Affilfont{\itshape\footnotesize}
\usepackage{booktabs}
\usepackage{todonotes}
%\presetkeys{todonotes}{inline}{}

%%%% MATHS
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{commath}
\usepackage{array}
\usepackage{calc}
\usepackage{longtable}
\usepackage{multirow}
\usepackage{physics}
\usepackage[squaren]{SIunits}
\usepackage{tensor}
\usepackage{upgreek}

%%%% GRAPHICS
\usepackage{pstricks}
\usepackage{graphicx}
\graphicspath{{figures/}}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{listings}
\usepackage[section]{placeins}

%%%% LISTINGS
\usepackage{listings}

%%%% TiKZ
%\usepackage[compat=1.1.0]{tikz-feynman}

%%%% FONTS etc
\usepackage[utf8]{inputenc}

%%%% LAYOUT
\usepackage[a4paper,pdfborder={0 0 0}]{hyperref}
\usepackage[format=hang,labelfont=bf,hypcap=true]{caption}
\usepackage{subfig}
\usepackage{sectsty}
\usepackage{relsize}
\usepackage[capitalise]{cleveref}
\usepackage{comment}

%\setlength{\parindent}{0mm}
\setlength{\voffset}{-1cm}
\setlength{\hoffset}{-1.75cm}
\setlength{\textwidth}{16.5truecm}
\setlength{\textheight}{24cm}
\setlength{\topmargin}{0mm}
\setlength{\headheight}{0mm}
\setlength{\headsep}{0mm}
\setlength{\parskip}{1mm}
\setlength{\mathindent}{2ex}

\let\spreprint\empty
\newcommand{\preprint}[1]{\def\spreprint{\protect#1}}
\let\sinstitute\empty
\newcommand{\institute}[1]{\def\sinstitute{\protect#1}}
\makeatletter
\renewcommand{\maketitle}{\begingroup
  \null\thispagestyle{empty}%
    \ifx\spreprint\empty
      \vskip 5ex
    \else
      \flushright\large\spreprint\vskip 2ex
    \fi
    \vskip 5ex
    \centering
      {\bfseries\Large\@title}\vskip 2ex
      \@author\vskip 2ex
      \ifx\sinstitute\empty
      \else
        {\large\sinstitute}
      \fi
    \vskip 5ex
  \endgroup
}
\makeatother
\renewenvironment{abstract}{\begin{center}
  \begin{minipage}[t]{0.75\textwidth}
  {\large\sffamily\bfseries Abstract}\newline%
}{\end{minipage}\end{center}\vskip 10ex}

%%%% CODE SHORTHANDS
\newcommand{\Comix}{C\protect\scalebox{0.8}{OMIX}\xspace}
\newcommand{\BlackHat}{B\protect\scalebox{0.8}{LACK}H\protect\scalebox{0.8}{AT}\xspace}
\newcommand{\Dire}{D\protect\scalebox{0.8}{IRE}\xspace}
\newcommand{\GoSam}{G\protect\scalebox{0.8}{O}S\protect\scalebox{0.8}{AM}\xspace}
\newcommand{\MCFM}{M\protect\scalebox{0.8}{CFM}\xspace}
\newcommand{\MadGraph}{M\protect\scalebox{0.8}{AD}G\protect\scalebox{0.8}{RAPH}\xspace}
\newcommand{\MadLoop}{M\protect\scalebox{0.8}{AD}L\protect\scalebox{0.8}{OOP}\xspace}
\newcommand{\MGaMC}{M\protect\scalebox{0.8}{AD}G\protect\scalebox{0.8}{RAPH}5\_\protect\scalebox{0.8}{A}M\protect\scalebox{0.8}{C}@N\protect\scalebox{0.8}{LO}\xspace}
\newcommand{\NJet}{N\protect\scalebox{0.8}{JET}\xspace}
\newcommand{\OpenLoops}{O\protect\scalebox{0.8}{PEN}L\protect\scalebox{0.8}{OOPS}\xspace}
\newcommand{\Pythia}{P\protect\scalebox{0.8}{YTHIA}\xspace}
\newcommand{\Rambo}{R\protect\scalebox{0.8}{AMBO}\xspace}
\newcommand{\Recola}{R\protect\scalebox{0.8}{ECOLA}\xspace}
\newcommand{\Sherpa}{S\protect\scalebox{0.8}{HERPA}\xspace}
\newcommand{\Vincia}{V\protect\scalebox{0.8}{INCIA}\xspace}

%%% NEW COMMANDS
\newcommand{\s}[1]{\ensuremath{s_{#1}}}
\newcommand{\D}{\ensuremath{\,\text{d}}}
\newcommand{\expo}[1]{\ensuremath{\,\text{e}^{#1}}}
\newcommand{\eulergamma}{\ensuremath{\upgamma_\mathrm{E}}}
\newcommand{\Order}[1]{\ensuremath{\mathcal{O}\left(#1\right)}}
\newcommand{\CA}{\ensuremath{C_\mathrm{A}}}
\newcommand{\CF}{\ensuremath{C_\mathrm{F}}}
\newcommand{\TR}{\ensuremath{T_\mathrm{R}}}
\newcommand{\nF}{\ensuremath{n_\mathrm{F}}}
\newcommand{\alphaS}{\ensuremath{\alpha_{\mathrm{s}}}}
\newcommand{\gS}{\ensuremath{g_{\mathrm{s}}}}
\newcommand{\muF}{\ensuremath{\mu}_\mathrm{F}}
\newcommand{\muR}{\ensuremath{\mu}_\mathrm{R}}
\newcommand{\muFSq}{\ensuremath{\mu}_\mathrm{F}^2}
\newcommand{\muRSq}{\ensuremath{\mu}_\mathrm{R}^2}
\newcommand{\BT}{{\mathbf{T}}}
\newcommand{\BI}{{\mathbf{I}}}
\newcommand{\CalA}{{\mathcal{A}}}
\newcommand{\CC}{{\mathcal{C}}}
\newcommand{\CI}{{\mathcal{I}}}
\newcommand{\CP}{{\mathcal{P}}}
\newcommand{\CS}{{\mathcal{S}}}
\newcommand{\CV}{{\mathcal{V}}}
\newcommand{\CM}{{\mathcal{M}}}
\newcommand{\UI}{{\mathrm{I}}}
\renewcommand{\Re}{\ensuremath{\mathrm{\,Re}}}

